Tradeoffs between convergence rate and noise amplification for momentum-based accelerated optimization algorithms

We study momentum-based first-order optimization algorithms in which the iterations utilize information from the two previous steps and are subject to an additive white noise. This setup uses noise to account for uncertainty in either gradient evaluation or iteration updates, and it includes Polyak's heavy-ball and Nesterov's accelerated methods as special cases. For strongly convex quadratic problems, we use the steady-state variance of the error in the optimization variable to quantify noise amplification and identify fundamental stochastic performance tradeoffs. Our approach utilizes the Jury stability criterion to provide a novel geometric characterization of conditions for linear convergence, and it reveals the relation between the noise amplification and convergence rate as well as their dependence on the condition number and the constant algorithmic parameters. This geometric insight leads to simple alternative proofs of standard convergence results and allows us to establish ``uncertainty principle'' of strongly convex optimization: for the two-step momentum method with linear convergence rate, the lower bound on the product between the settling time and noise amplification scales quadratically with the condition number. Our analysis also identifies a key difference between the gradient and iterate noise models: while the amplification of gradient noise can be made arbitrarily small by sufficiently decelerating the algorithm, the best achievable variance for the iterate noise model increases linearly with the settling time in the decelerating regime. Finally, we introduce two parameterized families of algorithms that strike a balance between noise amplification and settling time while preserving order-wise Pareto optimality for both noise models.

==> commandsHesam.tex <==
% =============================================================================
% Hesameddin Mohammdi
% The basic set of user-defined commands
% =============================================================================

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand*\mystrut[1]{\vrule width0pt height0pt depth#1\relax}
\DeclareMathOperator{\EX}{\mathbb{E}}
\newcommand{\hmmargin}[1]{\marginnote{\color{blue!80!white}\tiny\ttfamily{HM:} #1}}

\newcommand{\Z}{\mathbb{Z}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\DefinedAs}[0]{\mathrel{\mathop:}=}
\newcommand{\AsDefined}[0]{=\mathrel{\mathop:}}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\logdet}{log\,det}
\DeclareMathOperator*{\vecform}{vec}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\maximize}{maximize}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\subject}{subject~to}
\DeclareMathOperator*{\rank}{rank}

\newcommand{\new}{{\rm new}}
\newcommand{\old}{{\rm old}}
\newcommand{\barp}{{\bar p}}
\newcommand{\Diag}{{\rm Diag}\;}
\newcommand{\CP}{{\cal P}}
\newcommand{\rmCAP}{{\rm CAP}}
\newcommand{\epc}{\hspace{1pc}}
\newcommand{\gap}{\vspace{0.1in}}
\newcommand{\Mbld}{{\mbox{\bf M}}}
\newcommand{\Xbld}{{\mbox{\bf X}}}
\newcommand{\qbld}{{\mbox{\bf q}}}
\newcommand{\scmax}{{\rm {\scriptstyle max}}}
\newcommand{\sign}{{\rm {\scriptstyle sign}}}
\newcommand{\scdia}{{\rm {\scriptstyle dia}}}
\newcommand{\sclow}{{\rm {\scriptstyle low}}}
\newcommand{\scupp}{{\rm {\scriptstyle upp}}}

\newcommand{\abs}[1]{\lvert #1 \rvert} 




\newcommand{\tc}{\textcolor}
\newcommand{\vsp}{\vspace*{0.15cm}}
\newcommand{\atan}{\mathrm{atan}}

\newtheorem{mydef}{Definition}
\newtheorem{mythm}{Theorem}
\newtheorem{myprop}{Proposition}
\newtheorem{mylem}{Lemma}
\newtheorem{myrem}{Remark}
\newtheorem{myass}{Assumption}
\newtheorem{myfp}{Feasibility Problem}
\newtheorem{mycor}{Corollary}

\newcommand{\one}{\mathds{1}}
\newcommand{\qedsymbol}{$\blacksquare$}
\DeclareMathOperator*{\Null}{Null}

\newcommand{\Lf}{L}
\newcommand{\mf}{m}







